Benchmarking Neural Network Generalization for Grammar Induction

How well do neural networks generalize? Even for grammar induction tasks, where the target generalization is fully known, previous works have left the question open, testing very limited ranges beyond the training set and using different success criteria. We provide a measure of neural network generalization based on fully specified formal languages. Given a model and a formal grammar, the method assigns a generalization score representing how well a model generalizes to unseen samples in inverse relation to the amount of data it was trained on. The benchmark includes languages such as $a^nb^n$, $a^nb^nc^n$, $a^nb^mc^{n+m}$, and Dyck-1 and 2. We evaluate selected architectures using the benchmark and find that networks trained with a Minimum Description Length objective (MDL) generalize better and using less data than networks trained using standard loss functions. The benchmark is available at https://github.com/taucompling/bliss.

==> sandbox.tex <==

\section{The \textsc{BLISS} benchmark}

To make the human-ANN generalization gap concrete and measurable, and to encourage work in this direction, we release the Benchmark for Language Induction from Short Sequences (\textsc{bliss}).  
The benchmark contains training and test sets for the tasks described below. 

\begin{itemize}
    \item We designed the benchmark so that it embody the two main challenges for ANNs discussed above: their shortcoming in generalizing from little data, and the inability to prove in full generality that they are correct for any string in the relevant language (as can be done, in contrast, by induction in discrete and symbolic systems such as finite-state automata). This is done by keeping the training sets small, while considerably enlarging the test sets beyond previous probes in the literature. 
    
    \item However, it is important to emphasize that even success on extremely long test strings cannot guarantee that a model has mastered a task: even when a model reaches 100\% accuracy up to length $N$, it might still be wrong at $N+1$. (as was shown for LSTMs in \citealp{weiss:2018}). Full provability for neural networks remains extremely rare.

    \item Among connectionist models, we are aware of only one model to date that addresses both these challenges: \citet{lan:2022a} developed a recurrent neural network (RNN) that is optimized using a minimum description length (MDL) objective, essentially minimizing the network's error and the architecture's size at the same time (MDLRNN). 
    Minimizing the network's architecture forces it to generalize better and results in very small networks, making it possible to rigorously prove that networks generalize correctly to any string in a language. 

    \item MDLRNNs were shown to correctly learn most of the tasks in the benchmark presented below, including correctness proofs by induction. Because the MDL objective is not differentiable, which makes it incompatible with gradient-based methods such as backpropagation, MDLRNNs are trained using a non-standard optimization method that makes it possible to mutate the network's architecture at the same time (a genetic algorithm). While effective for simple languages such as $A^nB^n$, the approach failed to reach perfect results for languages which require the computational power of pushdown automata (PDAs, i.e., a stack), such as Dyck-2; these seem to require a better coverage of the hypothesis space. While \citet{lan:2022} show that an exhaustive enumeration of the hypothesis space based on MDL would result in perfect networks, solving the stack-requiring tasks in our benchmark remains unsolved for automatic methods. Moreover, liberated from differentiability constraints, this work used non-standard non-differentiable activation functions such as step functions (\textit{sign}, \textit{floor}, and \textit{modulo}). In Section~?? we test whether MDLRNN are competitive with standard architectures when limited to differentiable activations.
    
\end{itemize}


\subsection{Tasks}

Our benchmark is split into two types of targets: formal languages and simple arithmetic tasks (addition and multiplication). 

\subsubsection{Formal languages}

Learning of formal languages has played an important role in generative linguistics since its conception (Chomsky 1957), following the assumption that if a model cannot learn a formal language that is equally or less complex than natural language, it will not be able to learn human language either. With the rise of highly capable ANNs, interest has grown in inspecting these models' capabilities with respect to formal languages of different complexities (\citealp{weiss:2018}, ...?). 

However, previous works have overlooked several important ways in which human learning is unique: first, humans learn these languages perfectly and in full generality: when interrogated, they are able to explicitly describe the rules or grammars they had learned, and it is easy to verify that these are correct for \textit{any} $n$. No ANN that we know of is yet able to achieve this: ANNs' reliance on gradient-based training forces the use of continuous activation functions and prevents models from expressing discrete and symbolic grammars that are fundamental to human thought (ref); moreover, these models' large architectures lead to memorization of inputs at the expense of generalization, while at the same time making it hard to inspect their acquired knowledge. These pathologies lead to models that are not discrete, general, or interpretable -- three important ways in which they differ from humans.

% tend to memorize their inputs instead of generalizing, eventually providing wrong predictions for larger values of $n$; and they are often very hard to inspect and 

% We know of no connectionist model that is able to do that: these models are often too large to inspect, and extracting . Second, human explanations of these t provide discrete

Second, and more importantly to our current discussion, humans learn these tasks very quickly and based on very little data. This can be shown informally through simple introspection as in Section~\ref{sec:intro}, as well as empirically: works that have tested formal language learning in non-human primates have also tested humans on the same tasks. \citet{fitch:2004} found that humans learn the regular language $(AB)^n$ and the context-free language $A^nB^n$ after seeing 60 sequences as short as 4 and 6 characters, respectively. \citet{malassis:2020} found that the context-free palindrome language ($ww^R$) and the context-sensitive repeat language ($ww$) were learned perfectly based on no more than 64 sequences of length 4.\textbf{TODO add Ferringo 2020.}\footnote{Non-human primates, on the other hand, require significantly longer training time and exposure, do not acquire languages beyond context-free \citep{malassis:2020}, and naturally cannot provide proof of full generalization to any $n$ because of communication barriers -- thus sharing many of the same pathologies as current ANNs.} 

These results can serve as a baseline for sequence lengths and dataset sizes in our benchmark. For the languages mentioned above, then, it is safe to set $n$ as low as 4, and the training set data sizes at around 60. However, we make the challenge more lenient in terms of training set sizes because of two reasons. First, the lack of human data for all the tasks at hand makes it hard to set exact sizes across the board. We note however that even a training set containing a few hundred sequences is still considerably smaller than the ones used in any previous work that we're aware of: most empirical tests for ANNs to date were interested in squeezing the best accuracy out of models, often ignoring the departure from human-plausible datasets. Table~??? summarizes the training set sizes and lengths used in previous works. 
% (and failing to reach human performance even then). 

Second, \textbf{TODO}.

We include classical formal languages of increasing complexity: regular ($(AB)^n$), context-free ($A^nB^n$, $A^nB^mC^{n+m}$, Dyck-1, and the mirror/palindrome language $ww^R$), and context-sensitive ($A^nB^nC^n$, $A^nB^nC^nD^n$, Dyck-2, and the repeat language $ww$). 

Each of these complexity classes presents a challenge to ANNs in terms of learning. Regular languages can be represented using finite-state automata (FSA), but FSAs are discrete and symbolic formalisms while ANNs aren't, as discussed above. Context-free languages can be learned using a pushdown automaton, but ANNs struggle with such tasks unless explicitly equipped with specially designed differential stacks (\textbf{ref}). A particular family of languages crosses several classes of the complexity classes and contains languages that can be recognized using simple counting mechanisms: these are languages such as $A^nB^n$ and Dyck-1, for which a simple counter suffices. Despite previous works claiming that models such as RNNs such as LSTM are able to implement counting mechanisms thanks to architectural choices (Gers & Schimdhuber 2001), recent works have shown that these counters are not general and break at relatively low values (TODO refs Weiss 2018, El-Nagger 2022). We emphasize that this fragility cannot be explained by technical limitations, such as finite precision: LSTM generalization breaks for values as low as XXX; even low precision implementation such as 16-bit floats are able to store much larger values.\footnote{Modern implementations such as PyTorch use 32-bit float precision by default, which can store values up to at least $3\times 10^{38}$.}

The formal language tasks are presented in a language modeling setting, in which the model's goal is to assign a probability distribution to the next character in a sequence given its prefix. Following \citet{gers:2001}, each sequence starts with a start-of-sequence symbol, and ends with an end-of-sequence symbol.


    % Second, 
    
    % However, we emphasize that the exact number does not matter, since we are interested in two human characteristics 
    
    % it is possible for an artificial model 
    
    % because of the lack of empirical data of human performance for all the tasks we describe below, and given a possible human-machine performance gap we describe below, we release the benchmark in three increasing sizes: \textsc{bliss-Small}, \textsc{bliss-Medium}, \textsc{bliss-Large}. All three sizes are still considerably small than any training size used for current artificial networks.  

    % \item Humans also seem to need relatively little exposure to learn these tasks -- XX and YY exposures for $(AB)^n$ and $A^nB^n$, respectively.
    
    % In terms of training set sizes, which roughly correspond to the number of exposures humans need to learn a task, 

    % \item Beyond sequence length, how many samples should each dataset contain? Again, this can be approximated by the number of samples that humans require in order to learn the languages under discussion. 
    
    % For languages such as the palindrome and mirror languages ($ww^R$ and $ww$), humans learn from sequences as short as 4 characters long \citep{malassis:2020}. Similarly for $(AB)^n$ and $A^nB^n$ humans learn well from sequences lengths 4 and 6 respectively \citep{fitch:2004}.

\subsubsection{Binary addition and multiplication}

\begin{itemize}
    \item The addition and multiplication tasks the model reads both inputs simultaneously and outputs the result bit by bit.
\end{itemize}



\section{Preliminary evaluation}

\begin{itemize}
    \item We test \textsc{bliss} on the following modern ANNs: recurrent neural networks (RNNs) of the LSTM architecture \citep{hochreiter:1997}, a Transformer model (GPT-x?), and RNNs trained using a Minimum Descrition Length  (MDLRNN; \citealp{lan:2022a}). 

    \item Results: TODO
    
\end{itemize}

\section{Summary}

\begin{itemize}
    \item TODO
\end{itemize}
